Inference under Covariate-Adaptive Randomization with Multiple Treatments

This paper studies inference in randomized controlled trials with covariate-adaptive randomization when there are multiple treatments. More specifically, we study inference about the average effect of one or more treatments relative to other treatments or a control. As in Bugni et al. (2018), covariate-adaptive randomization refers to randomization schemes that first stratify according to baseline covariates and then assign treatment status so as to achieve balance within each stratum. In contrast to Bugni et al. (2018), we not only allow for multiple treatments, but further allow for the proportion of units being assigned to each of the treatments to vary across strata. We first study the properties of estimators derived from a fully saturated linear regression, i.e., a linear regression of the outcome on all interactions between indicators for each of the treatments and indicators for each of the strata. We show that tests based on these estimators using the usual heteroskedasticity-consistent estimator of the asymptotic variance are invalid; on the other hand, tests based on these estimators and suitable estimators of the asymptotic variance that we provide are exact. For the special case in which the target proportion of units being assigned to each of the treatments does not vary across strata, we additionally consider tests based on estimators derived from a linear regression with strata fixed effects, i.e., a linear regression of the outcome on indicators for each of the treatments and indicators for each of the strata. We show that tests based on these estimators using the usual heteroskedasticity-consistent estimator of the asymptotic variance are conservative, but tests based on these estimators and suitable estimators of the asymptotic variance that we provide are exact. A simulation study illustrates the practical relevance of our theoretical results.

==> Auxiliary_MCsimus.tex <==
%!TEX root = ../covariateadaptive.tex
\section{Additional Simulations} \label{app:moresimus}

In this section, we examine the finite-sample performance of several different tests of \eqref{eq:nullalt}, including those introduced in Section \ref{sec:main}, with the same simulation study from Section \ref{sec:simulations}. The only difference here is that $\pi=0.3$, as opposed to $\pi=1/2$.

Table \ref{tab:pi.g2} displays the results of the simulation study for $(\gamma,\sigma_1)\in\{(2,1),(2,\sqrt{2})\}$ and Table \ref{tab:pi.g4} displays the results of the simulation study for $(\gamma,\sigma_1)\in\{(4,1),(4,\sqrt{2})\}$ .  In the `SFE' column in both tables, the first number corresponds to homoskedasticity-only standard errors and the second number corresponds to the heteroskedasticity-robust standard errors.  We organize our discussion of the results by test:

\begin{itemize}
\item[] {\bf $t$-test}:  As expected in light of Theorem \ref{theorem:ttest} and Remark \ref{remark:conservative}, we see the two-sample $t$-test has rejection probability under the null hypothesis very close to the nominal level under simple random sampling, but has rejection probability under the null hypothesis strictly less than the nominal level under the more complicated randomization schemes.  

\item[] {\bf Na\"ive}: The results for the na\"ive permutation test are very similar to those for the two-sample $t$-test.

\begin{table}[t!] %seed 1000-1200
	\begin{center}
	\scalebox{0.9}{\input{Appendix/MCTable.pi.g2.ordered.tex}}
	\end{center} 
	\caption{Parameter values: $\gamma=2$, $\sigma_1=1$ (left panel) and $\gamma=2$, $\sigma_1=\sqrt{2}$ (right panel).}
	\label{tab:pi.g2}
\end{table}

\begin{table}[t!] %seed 1000-1200
	\begin{center}
	\scalebox{0.9}{\input{Appendix/MCTable.pi.g4.ordered.tex}}
	\end{center} 
	\caption{Parameter values: $\gamma=4$, $\sigma_1=1$ (left panel) and $\gamma=4$, $\sigma_1=\sqrt{2}$ (right panel).}
	\label{tab:pi.g4}
\end{table}

\item[] {\bf Reg}: The usual $t$-test (on the coefficient on treatment assignment) in a linear regression of outcomes $Y_i$ on treatment assignment $A_i$ and covariates $Z_i$ using heteroskedasticity-robust standard errors has rejection probability under the null hypothesis very close to the nominal level for Model 1. For all other models, the rejection probability of the test under the alternative hypothesis is lower than that of some of the other tests considered below.
\item[] {\bf SYZ}: For most specifications, the bootstrap-based test proposed by \cite{shao/yu/zhong:10} has rejection probability under the null hypothesis very close to the nominal level, though in some instances the rejection probability under the null hypothesis exceeds the nominal level.  
\item[] {\bf CAP}: As expected in light of Theorem \ref{theorem:cap}, when $\pi=0.3$ the covariate-adaptive permutation test has rejection probability under the null hypothesis above the nominal level, specially when $\sigma_1\ne \sigma_0$. 
\item[] {\bf SFE}: As expected in light of Theorem \ref{theorem:strata}, the $t$-test with strata fixed effects has rejection probability under the null hypothesis very close to the nominal level in nearly all specifications, provided that heteroskedasticity-robust standard errors are used. 
\end{itemize}

==> Table2.S10.pi3.g2.s1.tex <==
%!TEX root = ../expensivecar.tex
% Seed x3210
{\small 
\begin{tabular}{cl|cccccccc|ccccccc}
    \hline\hline
	\multicolumn{2}{c}{} & \multicolumn{7}{c}{Rejection rate under null - $\theta=0$}
           &\multicolumn{1}{c}{} & \multicolumn{7}{c}{Rejection rate under alternative - $\theta=0.2$} \\  
   \multicolumn{2}{c}{} & \multicolumn{3}{c}{SAT} & & \multicolumn{3}{c}{SFE} & \multicolumn{1}{c}{}& \multicolumn{3}{c}{SAT} & & \multicolumn{3}{c}{SFE}  \\ \cline{3-5} \cline{7-9} \cline{11-13}\cline{15-17}
       M  & \multicolumn{1}{c}{CAR} & HO & HC & NEW & & HO & HC & \multicolumn{1}{c}{NEW}& \multicolumn{1}{c}{} &HO & HC & NEW & & HO & HC & \multicolumn{1}{c}{NEW} \\
\hline 
1 & SRS & 4.63 & 4.75 & 4.70 & & 4.52 & 4.57 & 4.59 & & 79.26 & 79.66 & 79.60 & & 79.77 & 79.81 & 79.93 \\ 
  & SBR & 5.02 & 5.15 & 5.05 & & 5.02 & 5.00 & 5.03 & & 79.73 & 79.81 & 79.65 & & 79.71 & 79.55 & 79.71\\ 
\hline
2 & SRS & 11.49& 11.81& 4.91 & & 8.49 & 5.04 & 5.06 & & 73.63 & 74.11 & 58.31 & & 58.32 & 49.65 & 49.73  \\ 
  & SBR & 12.28& 12.63& 4.50 & & 4.89 & 2.57 & 4.61 & & 74.20 & 74.70 & 58.41 & & 59.73 & 48.70 & 59.29 \\ 
\hline
3 & SRS & 14.28& 14.74& 5.26 & & 9.05 & 5.15 & 5.19 & & 78.11 & 78.51 & 62.03 & & 61.89 & 51.83 & 51.92  \\ 
  & SBR & 13.56& 14.12& 4.55 & & 5.02 & 2.17 & 4.87 & & 78.38 & 78.92 & 61.56 & & 62.95 & 51.28 & 62.71  \\ 
\hline
4 & SRS & 32.39& 29.96& 5.10 & & 12.14& 5.20 & 5.23 & & 77.30 & 75.87 & 39.53 & & 43.95 & 28.28 & 28.39  \\ 
  & SBR & 32.33& 29.99& 4.84 & & 5.66 & 1.55 & 4.96 & & 77.18 & 75.35 & 38.97 & & 41.38 & 22.08 & 39.16 \\ 
\hline \hline
\end{tabular}} 




==> Table2B.S10.pi3.g2.s1.tex <==
%!TEX root = ../expensivecar.tex
% Seed x3210
{\small 
\begin{tabular}{cl|cccccccc|ccccccc}
    \hline\hline
	\multicolumn{2}{c}{} & \multicolumn{7}{c}{Rejection rate under null - $\theta=0$}
           &\multicolumn{1}{c}{} & \multicolumn{7}{c}{Rejection rate under alternative - $\theta=1/2$} \\  
   \multicolumn{2}{c}{} & \multicolumn{3}{c}{SAT} & & \multicolumn{3}{c}{SFE} & \multicolumn{1}{c}{}& \multicolumn{3}{c}{SAT} & & \multicolumn{3}{c}{SFE}  \\ \cline{3-5} \cline{7-9} \cline{11-13}\cline{15-17}
       M  & \multicolumn{1}{c}{CAR} & HO & HC & NEW & & HO & HC & \multicolumn{1}{c}{NEW}& \multicolumn{1}{c}{} &HO & HC & NEW & & HO & HC & \multicolumn{1}{c}{NEW} \\
\hline 
1 & SRS & 4.63 & 4.75 & 4.70 & & 4.52 & 4.57 & 4.59 & & 79.26 & 79.66 & 79.60 & & 79.77 & 79.81 & 79.93 \\ 
  & SBR & 5.02 & 5.15 & 5.05 & & 5.02 & 5.00 & 5.03 & & 79.73 & 79.81 & 79.65 & & 79.71 & 79.55 & 79.71\\ 
\hline
2 & SRS & 11.49& 11.81& 4.91 & & 8.49 & 5.04 & 5.06 & & 73.63 & 74.11 & 58.31 & & 58.32 & 49.65 & 49.73  \\ 
  & SBR & 12.28& 12.63& 4.50 & & 4.89 & 2.57 & 4.61 & & 74.20 & 74.70 & 58.41 & & 59.73 & 48.70 & 59.29 \\ 
\hline
3 & SRS & 14.28& 14.74& 5.26 & & 9.05 & 5.15 & 5.19 & & 78.11 & 78.51 & 62.03 & & 61.89 & 51.83 & 51.92  \\ 
  & SBR & 13.56& 14.12& 4.55 & & 5.02 & 2.17 & 4.87 & & 78.38 & 78.92 & 61.56 & & 62.95 & 51.28 & 62.71  \\ 
\hline
4 & SRS & 32.39& 29.96& 5.10 & & 12.14& 5.20 & 5.23 & & 77.30 & 75.87 & 39.53 & & 43.95 & 28.28 & 28.39  \\ 
  & SBR & 32.33& 29.99& 4.84 & & 5.66 & 1.55 & 4.96 & & 77.18 & 75.35 & 38.97 & & 41.38 & 22.08 & 39.16 \\ 
\hline \hline
\end{tabular}} 




==> Table4.S10.pi7.g2.s1.tex <==
%!TEX root = ../expensivecar.tex
% Seed x3110 and 70x4 %\cmidrule{3-5}
{\small 
\begin{tabular}{cl|cccccccc|ccccccc}
    \hline\hline
	\multicolumn{2}{c}{} & \multicolumn{7}{c}{Rejection rate under null - $\theta=0$}
           &\multicolumn{1}{c}{} & \multicolumn{7}{c}{Rejection rate under alternative - $\theta=0.2$} \\  
   \multicolumn{2}{c}{} & \multicolumn{3}{c}{SAT} & & \multicolumn{3}{c}{SFE} & \multicolumn{1}{c}{}& \multicolumn{3}{c}{SAT} & & \multicolumn{3}{c}{SFE}  \\ \cline{3-5} \cline{7-9} \cline{11-13}\cline{15-17}
       M  & \multicolumn{1}{c}{CAR} & HO & HC & NEW & & HO & HC & \multicolumn{1}{c}{NEW}& \multicolumn{1}{c}{} &HO & HC & NEW & & HO & HC & \multicolumn{1}{c}{NEW} \\
\hline 
1 & SRS & 5.02 & 5.21 & 5.18 & & 4.91 & 4.95 & 4.96 & & 78.75 & 79.16 & 79.12 & & 78.97 & 79.12 & 79.18 \\ 
  & SBR & 5.24 & 5.29 & 5.30 & & 5.18 & 5.25 & 5.30 & & 80.47 & 80.77 & 80.66 & & 80.39 & 80.57 & 80.68  \\ 
\hline
2 & SRS & 12.51 & 12.71 & 4.86 & & 8.57 & 4.96 & 5.00 & & 74.54 & 74.63 & 58.24 & & 58.86 & 48.90 & 49.00 \\ 
  & SBR & 12.77 & 12.82 & 5.48 & & 5.23 & 2.69 & 5.50 & & 75.26 & 75.07 & 59.85 & & 58.38 & 48.39 & 59.14 \\ 
\hline
3 & SRS & 14.10 & 14.08 & 4.92 & & 8.74 & 4.82 & 4.86 & & 79.59 & 79.55 & 63.07 & & 63.19 & 52.76 & 52.82 \\ 
  & SBR & 14.51 & 14.55 & 5.58 & & 5.30 & 2.70 & 5.49 & & 80.23 & 80.22 & 64.26 & & 62.64 & 51.65 & 63.36 \\ 
\hline
4 & SRS & 30.08 & 33.38 & 5.07 & & 12.40& 5.55 & 5.56 & & 75.56 & 77.45 & 41.08 & & 43.15 & 28.88 & 28.95 \\ 
  & SBR & 30.09 & 32.96 & 5.56 & & 4.66 & 1.35 & 5.00 & & 75.88 & 77.89 & 43.37 & & 40.59 & 24.49 & 43.23  \\ 
\hline \hline
\end{tabular}} 

  
 

 
  
   
 
 
 

   
  


==> Table4B.S10.pi7.g2.s1.tex <==
%!TEX root = ../expensivecar.tex
% Seed x3110 and 70x4 %\cmidrule{3-5}
{\small 
\begin{tabular}{cl|cccccccc|ccccccc}
    \hline\hline
	\multicolumn{2}{c}{} & \multicolumn{7}{c}{Rejection rate under null - $\theta=0$}
           &\multicolumn{1}{c}{} & \multicolumn{7}{c}{Rejection rate under alternative - $\theta=0.2$} \\  
   \multicolumn{2}{c}{} & \multicolumn{3}{c}{SAT} & & \multicolumn{3}{c}{SFE} & \multicolumn{1}{c}{}& \multicolumn{3}{c}{SAT} & & \multicolumn{3}{c}{SFE}  \\ \cline{3-5} \cline{7-9} \cline{11-13}\cline{15-17}
       M  & \multicolumn{1}{c}{CAR} & HO & HC & NEW & & HO & HC & \multicolumn{1}{c}{NEW}& \multicolumn{1}{c}{} &HO & HC & NEW & & HO & HC & \multicolumn{1}{c}{NEW} \\
\hline 
1 & SRS & 5.02 & 5.21 & 5.18 & & 4.91 & 4.95 & 4.96 & & 78.75 & 79.16 & 79.12 & & 78.97 & 79.12 & 79.18 \\ 
  & SBR & 5.24 & 5.29 & 5.30 & & 5.18 & 5.25 & 5.30 & & 80.47 & 80.77 & 80.66 & & 80.39 & 80.57 & 80.68  \\ 
\hline
2 & SRS & 12.51 & 12.71 & 4.86 & & 8.57 & 4.96 & 5.00 & & 74.54 & 74.63 & 58.24 & & 58.86 & 48.90 & 49.00 \\ 
  & SBR & 12.77 & 12.82 & 5.48 & & 5.23 & 2.69 & 5.50 & & 75.26 & 75.07 & 59.85 & & 58.38 & 48.39 & 59.14 \\ 
\hline
3 & SRS & 14.10 & 14.08 & 4.92 & & 8.74 & 4.82 & 4.86 & & 79.59 & 79.55 & 63.07 & & 63.19 & 52.76 & 52.82 \\ 
  & SBR & 14.51 & 14.55 & 5.58 & & 5.30 & 2.70 & 5.49 & & 80.23 & 80.22 & 64.26 & & 62.64 & 51.65 & 63.36 \\ 
\hline
4 & SRS & 30.08 & 33.38 & 5.07 & & 12.40& 5.55 & 5.56 & & 75.56 & 77.45 & 41.08 & & 43.15 & 28.88 & 28.95 \\ 
  & SBR & 30.09 & 32.96 & 5.56 & & 4.66 & 1.35 & 5.00 & & 75.88 & 77.89 & 43.37 & & 40.59 & 24.49 & 43.23  \\ 
\hline \hline
\end{tabular}} 

  
 

 
  
   
 
 
 

   
  

